Federated Learning for Face Recognition via Intra-subject Self-supervised Learning

Federated Learning (FL) for face recognition aggregates locally optimized models from individual clients to construct a generalized face recognition model. However, previous studies present two major challenges: insufficient incorporation of self-supervised learning and the necessity for clients to accommodate multiple subjects. To tackle these limitations, we propose FedFS (Federated Learning for personalized Face recognition via intra-subject Self-supervised learning framework), a novel federated learning architecture tailored to train personalized face recognition models without imposing subjects. Our proposed FedFS comprises two crucial components that leverage aggregated features of the local and global models to cooperate with representations of an off-the-shelf model. These components are (1) adaptive soft label construction, utilizing dot product operations to reformat labels within intra-instances, and (2) intra-subject self-supervised learning, employing cosine similarity operations to strengthen robust intra-subject representations. Additionally, we introduce a regularization loss to prevent overfitting and ensure the stability of the optimized model. To assess the effectiveness of FedFS, we conduct comprehensive experiments on the DigiFace-1M and VGGFace datasets, demonstrating superior performance compared to previous methods.

==> contents/3_3_ProposedMethod.tex <==
\subsection{Global update step}
The global update step is a process in which the server collects and aggregates the parameters of the global models trained by each client. Training only with positive data eliminates the advantage of training with negative data in contrastive learning. To address this limitation, we train the generalized facial features through a global parameter update using FedAvg\cite{mcmahan2017communication}. This step is summarized as follows:

\begin{equation}
w_g^{t+1} = \sum_{c=1}^{C}\frac{|D_c|}{\sum_{c=1}^{C}|D_c|}w_c^{t}
\end{equation}
\newline where $t$ means $t$th communication round, $t \in \{0, ..., T\}$. After updating the parameters of the global model, the model is broadcast to all clients.

==> contents/4_ConvergenceAnalysis.tex <==
\section{Convergence analysis}
In this section, we analyze the convergence of FedPS. To do the analysis, we first need to make some preliminary definitions. The point where the local model is trained is designated as e. (For example, $w^{e+1}$ means the model parameter that has completed the $e+1$th training.) We denote the loss function of FedPS as $F$.
\newline\textbf{Assumption 1. Lipschitz Smoothness.}\\
If the gradient of the local model of any client c is L-Lipschitz smooth, the following formula holds.

\vspace{-0.3cm}
\begin{equation}
||\nabla_pF(p_1,w) - \nabla_pF(p_{2},w) ||_2 <= L||p_{1}-p_{2}||_2
\end{equation}
\begin{equation}
||\nabla_wF(p,w_1) - \nabla_pF(p,w_{2}) ||_2 <= L||w_{1}-w_{2}||_2
\end{equation}
\newline\textbf{Assumption 2. Unbiased Gradient and Bounded Variance}
\newline The $w$ and $p$ parameters each use SGD as an optimization function, so they each have unbiased and bounded variance. The parameter update process using SGD is as follows:

\begin{equation}
p^{e+1} = p^{e} - \eta\nabla_pF(p^e, w^e)
\end{equation}
\begin{equation}
w^{e+1} = w^{e} - \eta\nabla_wF(p^e, w^e)
\end{equation}
\vspace{-0.3cm}
\newline Assuming that the amount of change in the parameter is within a certain range, the conditions are as follows:

\begin{equation}
||p^{e} - p^*||_2 <= \epsilon_p
\end{equation}
\begin{equation}
||w^{e} - w^*||_2 <= \epsilon_w
\end{equation}
\newline where $\epsilon_p$ and $\epsilon_w$ are positive value. With this assumption, updates to each parameter occur randomly within a certain range.
\newline\newline \textbf{Theorem 1. Convergence analysis}\\
Based on Assumption 1 and Assumption 2, a convergence analysis of FedPS can be performed as follows:

\begin{align}
||p^{e+1} - p^*||_2 <= \epsilon_p - \eta L\epsilon_w \\
||w^{e+1} - w^*||_2 <= \epsilon_w - \eta L\epsilon_p
\end{align}
\vspace{-0.5cm}
\newline Based on the above analysis, we confirm that the parameters of FedPS converge within the real number range.
\newline\newline \textbf{Proof 1.}\\
First, the change in the objective function is estimated using the distance between parameters as follows.
\begin{align}
    ||p^{e+1} - p^*||_2 = ||p^e - \eta\nabla_pF(p^e, w^e) - p^*||_2 \\
    = ||p^e - p^* - \eta\nabla_pF(p^e, w^e)||_2 \\
    = ||p^e - p^* - \eta(\nabla_pF(p^e, w^e) - \nabla_pF(p^*, w^*)||_2 \\
    <= ||p^e - p^*||_2 - \eta||(\nabla_pF(p^e, w^e) - \nabla_pF(p^*, w^*)||_2 \\ 
    <= ||p^e - p^*||_2 - \eta L||w^t-w^*||_2
\end{align}
\vspace{-0.5cm}
\newline Similar to the expansion process above, the same process is repeated for $w$ to obtain the follows:

\begin{equation}
||w^{e+1} - w^*||_2 <= ||w^e - w^*||_2 - \eta L||p^e-p^*||_2    
\end{equation}
\vspace{-0.3cm}
\newline Now, based on Hypothesis 2, we develop the following:

\begin{align}
||w^{e+1} - w^*||_2 <= ||w^e - w^*||_2 - \eta L||p^e-p^*||_2 \\
<= \epsilon_w - \eta L\epsilon_p \\
||p^{e+1} - p^*||_2 <= ||p^e - p^*||_2 - \eta L||w^e-w^*||_2 \\
<= \epsilon_p - \eta L\epsilon_w
\end{align}
\vspace{-0.3cm}
\newline Through this, Theorem 1 was proven.

==> contents/6_AblationStudy.tex <==
\begin{table}[!t]
\begin{center}
\resizebox{1.0\textwidth}{!}{\Huge
\begin{tabular}{lccc|cc}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Setup}}} & \multicolumn{3}{c|}{\textbf{Modules}}                                                  & \textbf{DigiFace-1M} & \textbf{VGGFace} \\ \cline{2-6} 
\multicolumn{1}{c|}{}                                & \multicolumn{1}{l|}{Regularize loss}             & \multicolumn{1}{l|}{Self-similarity score}     & Top K \& $\gamma$ & TPIR@FPIR=0.001  & TPIR@FPIR=0.001  \\ \hline
\multicolumn{4}{l|}{Centrally trained with PocketNet}                                                                                         & 0.9128             & 0.9806             \\ \hline
\multicolumn{1}{l|}{A}                               & \texttimes & \texttimes & \texttimes      & 0.9051             & 0.9645             \\
\multicolumn{1}{l|}{B}                               & \checkmark & \texttimes & \texttimes      & 0.9537             & 0.9902             \\
\multicolumn{1}{l|}{C}                               & \checkmark & \checkmark & \texttimes      & 0.9319             & 0.9884             \\
\multicolumn{1}{l|}{Ours(D)}                         & \checkmark & \checkmark & \checkmark      & 0.9794             & 0.9934             \\ \hline
\end{tabular}
}
\end{center}
\vspace{-0.2cm}
\caption{The TPIR performance for ablation studies}
\vspace{-0.3cm}
\label{tab:tab_abla}
\end{table}

\begin{figure*}[!t]
\centerline{\includegraphics[width=1.0\textwidth]{images/figure_abli.pdf}}
\vspace{-0.2cm}
\caption{Average similarity distribution of clients participated in federated learning}
\label{fig:fig_abla}
\vspace{-0.2cm}
\end{figure*}


\section{Ablation Studies}
Self-similarity learning defined in Equation \ref{eq:total}, improves the performance of personalized face recognition compared to previous approaches. We go further and check whether the proposed method reduces intra-class variation and analyze how the method affects performance. We set the participation rate at 0.7, and use PocketNet \cite{boutros2022pocketnet} as the pre-trained model. As shown in Figure \ref{fig:fig_abla} and Table \ref{tab:tab_abla}, we can see that the self-similarity method considering correlation shows superior performance compared to using the general entropy learning method and regularize loss has a significant impact on performance by preventing overfitting and bias. In particular, as shown in figure \ref{fig:fig_abla}, the proposed method has the smallest intersection of the positive similarity area and the negative similarity area. Through these results, we confirm that self-similarity learning reduces intra-class variance.
